On the Relationship between Refactoring Actions and Bugs: A Differentiated Replication

Software refactoring aims at improving code quality while preserving the system's external behavior. Although in principle refactoring is a behavior-preserving activity, a study presented by Bavota et al. in 2012 reported the proneness of some refactoring actions (e.g., pull up method) to induce faults. The study was performed by mining refactoring activities and bugs from three systems. Taking profit of the advances made in the mining software repositories field (e.g., better tools to detect refactoring actions at commit-level granularity), we present a differentiated replication of the work by Bavota et al. in which we (i) overcome some of the weaknesses that affect their experimental design, (ii) answer the same research questions of the original study on a much larger dataset (3 vs 103 systems), and (iii) complement the quantitative analysis of the relationship between refactoring and bugs with a qualitative, manual inspection of commits aimed at verifying the extent to which refactoring actions trigger bug-fixing activities. The results of our quantitative analysis confirm the findings of the replicated study, while the qualitative analysis partially demystifies the role played by refactoring actions in the bug introduction.

==> sections/original.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary of the Replicated Study}
\label{sec:original}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We replicate the work by Bavota \etal \cite{BavotaCLPOS12} titled \emph{When does a Refactoring Induce Bugs? An Empirical Study}. This section briefly summarizes their experimental design. We discuss and compare their findings with ours in the results discussion. 

The authors used \tool{Ref-Finder} \cite{PreteRSK10} to create a dataset of 12,922 refactorings validated by two Master students and performed between 63 releases of three Java systems, namely Apache Ant, ArgoUML, and Apache Xerces-J. While the authors know that a specific refactoring operation was performed on a file $F_j$ between the releases $R_i$ and $R_{i+1}$ of a given system, the exact commit in which the refactoring was implemented was unknown. 

Then, by mining the change history of the three subject systems, the authors identified bug-fixing commits as those in which the developers used specific lexical patterns in the commit note to indicate the fixing of a bug (\eg ``\emph{fixed issue \#ID}'', where ID was the id of an issue on the issue tracker of the mined system). 

Finally, for each bug-fixing commit, the authors identified its fix-inducing commits by using the SZZ algorithm \cite{}. Given a bug-fixing commit impacting a set of source code lines $S$, the SZZ algorithm uses the blame feature of versioning systems to identify the commits in which the last changes any line in $S$ occurred. These commits are marked as fix-inducing, meaning as those that have triggered the fixing activity.

Using the above described data, Bavota \etal assumed that a refactoring operation performed on file $F_j$ between $R_i$ and $R_{i+1}$ induced a fixing activity if a bug-inducing commit $c$ identified by the SZZ was performed on $F_j$ between $R_i$ and $R_{i+1}$. It is worth noting here the strong assumption made in the experimental design: Since the refactorings were captured between releases, it is not possible to know whether the refactoring was actually implemented in the bug-inducing commit $c$. This is the main limitations of the original study that we try to overcome in our replication.
